Integrating Probabilistic Trees and Causal Networks for Clinical and Epidemiological Data

Healthcare decision-making requires not only accurate predictions but also insights into how factors influence patient outcomes. While traditional Machine Learning (ML) models excel at predicting outcomes, such as identifying high risk patients, they are limited in addressing what-if questions about interventions. This study introduces the Probabilistic Causal Fusion (PCF) framework, which integrates Causal Bayesian Networks (CBNs) and Probability Trees (PTrees) to extend beyond predictions. PCF leverages causal relationships from CBNs to structure PTrees, enabling both the quantification of factor impacts and simulation of hypothetical interventions. PCF was validated on three real-world healthcare datasets i.e. MIMIC-IV, Framingham Heart Study, and Diabetes, chosen for their clinically diverse variables. It demonstrated predictive performance comparable to traditional ML models while providing additional causal reasoning capabilities. To enhance interpretability, PCF incorporates sensitivity analysis and SHapley Additive exPlanations (SHAP). Sensitivity analysis quantifies the influence of causal parameters on outcomes such as Length of Stay (LOS), Coronary Heart Disease (CHD), and Diabetes, while SHAP highlights the importance of individual features in predictive modeling. By combining causal reasoning with predictive modeling, PCF bridges the gap between clinical intuition and data-driven insights. Its ability to uncover relationships between modifiable factors and simulate hypothetical scenarios provides clinicians with a clearer understanding of causal pathways. This approach supports more informed, evidence-based decision-making, offering a robust framework for addressing complex questions in diverse healthcare settings.

==> extra.tex <==
\begin{abstract}
Healthcare decision-making is of paramount importance, as decisions profoundly impact patient well-being. In this context, interpretable and transparent AI models play a crucial role, fostering trust among both clinicians and patients. This work introduces the Probabilistic Causal Fusion (PCF), a novel interpretable AI approach leveraging the synergy between Causal Bayesian Networks (CBNs) and ensembles of Probability Trees (PTrees). PCF harnesses the causal order learned by the CBN to structure PTrees, capturing inherent causal relationships and enabling domain knowledge incorporation through counterfactuals.

Validated on three real-world healthcare case studies (MIMIC-IV, Framingham Heart Study, Diabetes), PCF achieves comparable prediction performance to benchmarks. These case studies were selected for their comprehensive and diverse clinical data, which encompass a wide range of variables critical for evaluating the effectiveness of the PCF in different medical contexts.  The true value of PCF lies beyond mere prediction. Unlike traditional models, PCF empowers clinicians with a comprehensive toolkit for exploring hypothetical interventions and counterfactual scenarios. This enhanced understanding of risk factors, interventions, and  variable interactions significantly enhances clinical decision-making.

Furthermore, PCF introduces a new avenue for collaboration and knowledge sharing through a centralised causal knowledge repository. Large hospitals with extensive datasets can develop CBNs to represent causal relationships and create pre-trained PCF models. These models can then be securely shared with smaller hospitals, promoting efficient knowledge transfer and collaborative decision-making in healthcare. This innovative paradigm enhances inter-institutional collaboration, leveraging the collective expertise to improve patient outcomes.

This work surpasses the limitations of interpretable AI development in healthcare. By enabling collaborative model building through centralised knowledge sharing, PCF fosters generalisability across diverse settings. This transformative potential holds significant promise for revolutionising healthcare delivery and ultimately, improving patient outcomes.
\end{abstract}

\subsection{Interventions}
Examining the effects of interventions on heart rate reveals interesting insights. When manipulating the heart rate to be less than or equal to 60 beats per minute ($do(heart\_rate = 0)$), we observe a noticeable increase in the percentage of patients with $los=1$. This finding aligns with medical literature that links very low heart rates (bradycardia) to underlying medical conditions often requiring extended ICU stays for investigation or treatment \cite{heartrate}. However, it's crucial to note that interventions on heart rate alone might not be a definitive factor in determining los. While a similar increase in $los=1$ is observed compared to interventions where heart rate remains above 60 bpm ($do(heart\_rate = 1)$), we also see a somewhat decrease in $los=1$ when ($do(heart\_rate = 2)$). This suggests that heart rate, in isolation, might not be the sole determinant of los. Other factors likely play a role in the complex interplay that influences hospital stay duration.

Similar observations are made when analysing the effects of interventions on urea nitrogen (UN) levels. Manipulating UN levels to be low $do(Urea\_Nitrogen = 0)$ results in a decrease in the proportion of patients with $los=1$. This aligns with existing medical knowledge, as low UN levels are often associated with low-protein intake and are generally not considered a cause for concern \cite{urea}. However, as the intervention values are increased $do(Urea\_Nitrogen = 1)$ and $do(Urea\_Nitrogen = 2)$, a trend emerges indicating a potential rise in the probability of $los=1$. While this increase is subtle, it is visually detectable by the red color in the box plots.

On the other hand, when red cell distribution width (RDW) is manipulated to be high ($do(RDW = 2)$), there is an increase in the percentage of patients with $los=1$. This observation is consistent with the existing literature, which suggests that increased RDW is closely associated with the risk of cardiovascular morbidity and mortality in patients with previous myocardial infarction \cite{tonelli2008relation}.

When we intervene by setting $do(Creatinine = 0)$, a notable increase occurs in the likelihood of observing $los=1$. Similarly, an elevation in respiration rate $do(respiration = 2)$ coincides with a heightened probability of $los=1$. This relationship is indicative of tachypnea in adults, characterised by a respiratory rate exceeding 20 breaths per minute, often necessitating further assessment and resulting in prolonged hospital stays \cite{Puskarich2017AssociationBP}. Additionally, it is noteworthy that intervening on temperature $do(temperature = 1)$, indicating mild fever, also leads to an elevated probability of observing $los=1$.

Concerning oxygen saturation levels, inadequate saturation ($do(saturation = 1)$) elicits a varied effect on $los=1$. However, interventions targeting other saturation levels $do(saturation = 0)$, $do(saturation = 2)$, $do(saturation = 3)$, $do(saturation = 4)$, and $do(saturation = 5)$ do not yield a discernible impact on los. Conversely, when manipulating glucose levels, an inverse response is observed, implying that these variables may indirectly influence los through intermediary factors rather than exerting a direct effect on los.

\section{Introduction}
Healthcare thrives on accurate diagnoses, effective interventions, and a nuanced understanding of potential outcomes. Traditional machine learning models primarily focus on prediction, falling short of the intricate requirements of clinical decision-making. Additionally, a lack of transparency in ``black-box'' models hinders their integration into patient care. Justification for treatment recommendations is paramount, and clinicians require models that explain their rationale for confident integration into patient care plans.

To overcome the limitations of traditional prediction-focused models, graphical models, particularly Causal Bayesian Networks (CBNs) and Probability Trees (PTrees), have emerged as powerful tools for unraveling complex causality patterns in healthcare \cite{sanchez2022causal,prosperi2020causal,rajput2022causal,ambags2023assisting}. These models provide a structured framework to capture and visualise the interdependencies among variables, offering a nuanced perspective on different factors influencing patient outcomes.

While both CBNs and PTrees fall under the umbrella of probabilistic graphical models, they serve distinct purposes. CBNs excel at capturing causal relationships within complex systems. Their directed acyclic graph (DAG) structure explicitly delineates causal dependencies between variables, empowering researchers to conduct causal inference, make informed decisions, and devise effective intervention strategies \cite{reason:Pearl09a}. PTrees, on the other hand, offer an intuitive representation of probabilistic relationships using nodes and branches. This hierarchical structure simplifies comprehension of complex probabilistic dependencies and facilitates reasoning about uncertainty, a common aspect of healthcare decision-making \cite{genewein2020algorithms}. This complementary nature motivates the development of the PCF pipeline, a novel interpretable approach introduced in this work.

The Probabilistic Causal Fusion (PCF) pipeline transcends the limitations of individual models by harnessing the complementary strengths of CBNs and PTrees. By leveraging the rich causal knowledge gleaned from the CBN, PCF informs the structure of an ensemble of PTrees. This critical step ensures that the modeled probabilistic dependencies faithfully reflect the underlying causal relationships inherent in the data, a key advantage absent in traditional methods. Traditionally, constructing a PTree is an iterative and often subjective process, heavily reliant on domain experts for variable ordering \cite{ambags2023assisting}. This dependence introduces limitations:
\begin{enumerate}
\item Subjectivity: domain knowledge can be biased or incomplete, potentially leading to suboptimal PTree structures;
\item Inefficiency: the iterative process can be time-consuming, especially for complex datasets;
\item Data Inconsistency: PTrees constructed solely on expert knowledge might not fully capture the relationships present in the data.
\end{enumerate}
Furthermore, by employing an ensemble learning approach, PCF mitigates the limitations associated with single PTrees, particularly their susceptibility to overfitting.

The PCF pipeline not only functions as a sophisticated modeling tool but also establishes a centralised causal knowledge repository, facilitating collaboration and knowledge exchange among healthcare institutions. It offers pre-trained PCF models and their underlying causal structures, empowering smaller institutions to leverage collective expertise. This collaborative ecosystem fosters the development of generalisable models applicable across diverse healthcare settings. Furthermore, seamless knowledge transfer through the repository enables continuous improvement, as institutions can refine models based on shared experiences and local data. Figure \ref{fig:illustration} summarises different steps of the proposed PCF pipeline.

\begin{figure*}
\centering
    \includegraphics[width=\textwidth]{ChangedVisualabstract.jpg}
    \caption{Different steps involved in the PCF pipeline. The first module addresses data pre-processing to shape the input required for the CBN. The next module involves generating individual CBNs and creating a model-averaging graph. Subsequently, the ensemble of PTrees is developed based on the variable order from the model-averaging graph. The final module involves evaluating the overall performance of the PCF pipeline.}
    \label{fig:illustration}
\end{figure*}

This work leverages the developed pipeline to facilitate prediction, intervention, and counterfactual analysis in three distinct clinical contexts. First, we aim to predict and elucidate how various factors influence the length of stay in the Intensive Care Unit (ICU). Second, the pipeline is employed to predict the risk of Chronic Heart Disease (CHD) in patients and to analyse the potential factors that could lessen the risk of CHD development. Finally, we utilise the pipeline to predict the risk of diabetes and to comprehend the influence of diverse risk factors on its development. 
Overall, the main contributions of this work are described as follows:
\begin{itemize}
\item We present a novel framework, Probabilistic Causal Fusion (PCF), that integrates Causal Bayesian Networks (CBNs) with Probability Trees (PTrees) to facilitate predictions, interventions, and counterfactual analysis in healthcare. This innovative integration addresses the subjectivity and time-consuming nature of traditional PTree construction by autonomously establishing variable order through CBNs.
\item By employing an ensemble of PTrees, our methodology improves predictive accuracy and robustness. This ensemble strategy effectively balances the trade-off between bias and variance, reducing the risk of overfitting and underfitting.
\item We introduce key methodological refinements in computing transition probabilities within the PTree framework. This includes partitioning data based on empirical marginal probabilities and utilising causal relationships learned from CBNs for more informed split decisions, enhancing the model’s predictive capabilities.
\item The effectiveness of the PCF framework is demonstrated through its application to multiple real-world healthcare datasets.
\end{itemize} 

The paper is structured as follows. Section \ref{method} delves into the details of the proposed pipeline, including its construction process. This section is further divided into subsections that elucidate the specific steps involved in its development.    The application of the pipeline to three distinct clinical case studies is described in Section \ref{casestudies}. Section \ref{results} presents the findings obtained through the pipeline's application. Finally, Section \ref{conclusion} includes the conclusive remarks.


